MLCask: Efficient Management of Component Evolution in Collaborative Data Analytics Pipelines

With the ever-increasing adoption of machine learning for data analytics, maintaining a machine learning pipeline is becoming more complex as both the datasets and trained models evolve with time. In a collaborative environment, the changes and updates due to pipeline evolution often cause cumbersome coordination and maintenance work, raising the costs and making it hard to use. Existing solutions, unfortunately, do not address the version evolution problem, especially in a collaborative environment where non-linear version control semantics are necessary to isolate operations made by different user roles. The lack of version control semantics also incurs unnecessary storage consumption and lowers efficiency due to data duplication and repeated data pre-processing, which are avoidable. In this paper, we identify two main challenges that arise during the deployment of machine learning pipelines, and address them with the design of versioning for an end-to-end analytics system MLCask. The system supports multiple user roles with the ability to perform Git-like branching and merging operations in the context of the machine learning pipelines. We define and accelerate the metric-driven merge operation by pruning the pipeline search tree using reusable history records and pipeline compatibility information. Further, we design and implement the prioritized pipeline search, which gives preference to the pipelines that probably yield better performance. The effectiveness of MLCask is evaluated through an extensive study over several real-world deployment cases. The performance evaluation shows that the proposed merge operation is up to 7.8x faster and saves up to 11.9x storage space than the baseline method that does not utilize history records.

==> cover_letter.tex <==
\newcommand{\comments}[2]{\noindent\underline{\textbf{Comment #1}}: \emph{#2}}
\newcommand{\response}[1]{\vspace{1mm}\noindent\textbf{RESPONSE}: #1\vspace{1mm}}
\newcommand{\revhighlight}[1]{\emph{\textbf{\uuline{#1}}}}
\pagestyle{empty}
\thispagestyle{empty}

% \newcommand{\question}[1]{}
\newcommand{\question}[1]{{\textcolor{blue}{(#1)}}}

\onecolumn

\centerline{\textbf{\Large Response to Reviewers' Comments}}
\vspace{10mm}

\begin{multicols}{2}

\setcounter{page}{1}

\noindent To PC co-chairs, meta reviewer, and reviewers:

\vspace{5mm}
We would like to thank the meta reviewer and reviewers for their thorough reviews and valuable comments, which indeed help us to improve the quality of this paper.
We have studied the comments carefully and have addressed all the comments.
We have sought the approval of PC co-chairs to include an additional co-author, Lei Zhu, to help with the new experiments.  He is also responsible for deploying \system{} in another major public hospital. This explains the addition.
%%done our best to incorporate as much as possible the insightful feedback and suggestions. 

In this cover letter, we first summarize the changes that we have made, and then provide detailed point-by-point responses to the concerns raised by each reviewer. 
For ease of reading, we have highlighted the major changes in the revised paper in {\color{blue} blue}.

\section*{Summary of Changes}

We have addressed all the mandatory revision items listed in the meta review, as well as other weak points and detailed comments of all three reviewers:

\begin{itemize}
    \item We have added experiments to compare \system{} with two state-of-the-art  open-source  systems, namely, ModelDB and MLflow in Section~\ref{exp-linear-version}. 
    Specifically, results on the total time, pipeline time composition and cumulative storage space are respectively shown in Fig.~\ref{fig: lv-time}, Fig.~\ref{fig: lv-breakdown}. and Fig.~\ref{fig: lv-storage}.
    More details can be found in the response of Reviewer \#3 W1.
    \item We have added more details to explain how a user would use this system in Section~\ref{sec: system design}. The details can be found in the response of Reviewer \#3 W2.
    \item We have reported our experience on the system deployment in a new Section~\ref{sec: discussion} "Discussion on System Deployment". More details can be found in the response of Reviewer \#3 W3.
    \item We have added more clarity on the revised paper by addressing the comments in Reviewer \#1 W1, Reviewer \#1 D1 - D5 and Reviewer \#2 D4 - D5. 
    The revised sections with respect to the comments are located at:

    Reviewer \#1 W1: Section~\ref{exp-pps}
    
    Reviewer \#1 D1: Section~\ref{sec: supporting non-linear version history}

    Reviewer \#1 D2: Section~\ref{sec: supporting non-linear version history}

    Reviewer \#1 D3: Section~\ref{sec: supporting non-linear version history}

    Reviewer \#1 D5: Fig.~\ref{fig: lv-breakdown} (i.e. original Fig. 7) 
    
    Reviewer \#2 D4: Section~\ref{sec: supporting non-linear version history}

    Reviewer \#2 D5: Section~\ref{sec: supporting non-linear version history}

    \item We have also addressed other weak points and detailed comments of all three reviewers, including Reviewer \#1 W2-W3, Reviewer \#3 D4-D6.
\end{itemize}

%\question{May consider reducing the expression of reviewers' comments later}

\section*{Response to Reviewer \#1}
\comments{W1}{Some details are not clear. 
In particular, I would like to learn more about how correct the assembly of previously used pipelines works. 
This information is also not discussed in the experiments. 
The authors only focus on performance without showing that the more resource efficient solution leads actually to desired results.}

\response{
In the experiment section~\ref{exp-pps}, we have added paragraph 5 to clarify that we provide two approaches for our pipeline search solutions. 
While the optimal approach based on pruning focuses on the pipeline performance, another approach, prioritized pipeline search, is a more resource efficient solution that could also lead to desired results.
The key idea of the prioritized pipeline search is to evaluate the most promising solutions according to the history within a limited time budget, which leads to lower computational costs.


%The appended paragraph is located at the end of Section~\ref{exp-pps}:
%"In summary, \system{} supports two pipeline search approaches: (i) optimal approach with pruning, and (ii) prioritized pipeline search. 
%Both approaches search for feasible pipeline solutions from the search space which involves all the nonlinear versions starting from the common ancestor. 
%The optimal approach can obtain the global optimal solution, because it evaluates all the feasible solutions within the search space after pruning. 
%In contrast, the prioritized pipeline search only evaluates the most promising solutions according to the history within a limited time budget. 
%However, the computational cost of the prioritized pipeline search is lower and resource efficient.
%Hence it may be a more practical solution."
}

\comments{W2}{
The baseline is not explained in detail. 
The authors only mention that non-linear semantics is not included but they don't say what is actually included and how the approach works. 
}

\response{
We have added more details of baseline systems, namely, ModelDB and MLflow, with respect to storage mechanism, reuse of intermediate results, and how they support reproducibility, query and comparison of machine learning models in subsection~\textbf{Baseline for Linear Versioning} of Section~\ref{exp-baseline}.


% "We compare \system{} against two state-of-the-art open-source systems, ModelDB~\cite{vartak2016modeldb} and MLflow~\cite{zaharia2018accelerating}. 
% The two baseline systems manage different model versions to support reproducibility.
% Users are provided tracking APIs to log parameters, code, and results in machine learning experiments so that they can query the details of different models and compare them.
% For these two systems, ModelDB does not offer automatic reuse of intermediate results and MLflow is able to reuse intermediate results. 
% The storage mechanism of both systems archives different versions of libraries and intermediate results into separate folders."


% Experiments that compare \system{} with these two baseline systems in terms of run time and storage size are also added in Section~\ref{exp-linear-version}.
}

\comments{W3}{It is not clear to which extent the non-linear character of the github is challenging and also it is not clear how its inclusion benefits the overall process. The latter could be clarified by addressing W2.}

\response{
The non-linear character of the github is challenging because the pipeline search space, which involves all the available component versions developed starting from the common ancestors, is typically
huge and could have multiple local optima.
We have added more clarification on this in paragraph 4 of subsection \textbf{Merge} in Section~\ref{sec: supporting non-linear version history} and at the beginning of Section~\ref{sec: optimizing version operations}.

Baseline systems, i.e., ModelDB and MLflow, are designed for the linear versioning.
Nevertheless, for branching and merging of updated pipelines, non-linear versioning is needed, which is provided by \system{}.
We have added more clarification on the benefits of non-linear versioning in Section~\ref{sec: discussion}.
}

\comments{D1}{The paper is quite verbose with regard to high-level goals. 
Most of it are repeated at various places. 
Especially the announcement of handling non-linear semantics. 
Instead I would go into a bit more detail to explain these concepts.
}

\response{
To reduce the redundancy on the explanation of handling non-linear semantics, we have removed the original Fig. 1 and its description in Section~\ref{sec: challenge}. This is now only discussed
%%This is because similar concepts in high-level are discussed 
in Section~\ref{sec: supporting non-linear version history}.
Moreover, to explain these concepts more clearly, we have added more details of merging two asynchronously updated pipelines with non-linear semantics, in subsection~\textbf{Merge} of Section~\ref{sec: supporting non-linear version history}.
}

\comments{D2}{
Figure 5 is not really explainable. 
You say that some components are not compatible, but can I see it apart from the color?
}

\response{
The pipeline search tree in Fig. 5 (Fig.~\ref{fig:pipeline-search-tree} of the revised version) is generated based on Fig. 4 (Fig.~\ref{fig:branch-merge} of the revised version). 

The nodes in green color already have checkpoints in the development history as depicted in Fig.~\ref{fig:branch-merge}.
The nodes in red color are not executable due to the incompatibility between pipeline components, which are determined by the compatibility information introduced in Section~\ref{sec: prun} together with the semantic version rule in paragraph 2 of Section~\ref{sec: version control of pipeline components}.
The remaining nodes in orange are those need to be executed.

These details are added in paragraph 10 of subsection~\textbf{Merge} in Section~\ref{sec: supporting non-linear version history}.


% The modified paragraph is located at Section~\ref{sec: supporting non-linear version history} at the topic \textbf{Merge}:

%"Fig.~\ref{fig:pipeline-search-tree} illustrates an example of a pipeline search tree.
%This pipeline search tree is generated according to the merge operation illustrated in Fig.~\ref{fig:branch-merge} between the two branches HEAD and MERGE HEAD. ... ... There are three types of nodes denoted with different colors: green, red, and orange. 
%The nodes in green color already have checkpoints in the development history starting from the common ancestor depicted in Fig.~\ref{fig:branch-merge}. 
%The nodes in red color are not executable due to the incompatibility between pipeline components, which are determined by the compatibility information introduced in Section~\ref{sec: prun}. 
%Finally, the nodes in orange, called feasible nodes, are the remaining nodes that need to be executed.
%The nodes in red and green colors will be further elaborated in Sections~\ref{sec: prun} and \ref{sec:reuseable} respectively."
}
%%% ooibc: need to repeat such statements, since they are marked in blue font.  Too "luo suo" is anooying.

\comments{D3}{
In Figure 5 you mention feasible nodes. What are those? Are these pipelines that do not exist in such form in the database? If so how do you generate them? This needs to be better clarified.
}

\response{
In Fig. 5 (Fig.~\ref{fig:pipeline-search-tree} of the revised paper), the feasible nodes in orange color refer to the only nodes that need to be executed in a pipeline search tree after pruning the green color nodes which are executed before and the red color nodes which are incompatible.

The above explanation in more details has been included in paragraph 10 of subsection~\textbf{Merge} in Section~\ref{sec: supporting non-linear version history}.

We have developed Algorithm~\ref{alg:traverse-and-execute} to prune the nodes which are executed before or incompatible and then execute the remaining orange color feasible nodes.

%"The nodes in green color already have checkpoints in the development history starting from the common ancestor depicted in Fig.~\ref{fig:branch-merge}. 
%The nodes in red color are not executable due to the incompatibility between pipeline components, which are determined by the compatibility information introduced in Section~\ref{sec: prun}. 
%Finally, the nodes in orange, called feasible nodes, are the remaining nodes that need to be executed."
}
%%% ooibc: again, why bother -- if leave in the paper, some will not read, but will pick up more incosistency here

\comments{D4}{
You say that the system is deployed at a hospital, which is great. But why not also publish the code?
}

\response{
% To prevent leaking the design concept of the system, we are not going to release the code before publishing a paper. 
% Furthermore, we will need to clean and refactor the code to improve the usability after lots of design works on the prototype.
The code will be released as part of Apache SINGA. 
However, there is a dependency (ForkBase storage engine) that can only be provided as executable for the time being. 
%%% zj: this answer is from the response to SIGMOD-2021, need to check this
}


\comments{D5}{
Figure 7 is really not readable.
}

\response{
We have updated the figure (Fig.~\ref{fig: lv-breakdown} of the revised paper).
}


\section*{Response to Reviewer \#2}
\comments{D4}{It has been said that the merge of recent versions of two components can result in a sub-optimal pipeline. An example would be helpful.}

\response{
We have added an example to show that the merge of recent versions of two components can result in a sub-optimal pipeline in paragraph 4 of subsection~\textbf{Merge} in Section~\ref{sec: supporting non-linear version history}.
The example shows that we cannot guarantee the recent versions of a component in a pipeline is still performing well after it is merged with another pipeline because it involves the updates of other components.

%"For the second reason, the na\"ive strategy does not guarantee optimal performance due to the complex coupling among pipeline components.
%In the two branches HEAD and MERGE HEAD of Fig.~\ref{fig:branch-merge}, the three updated components Data Cleansing, Feature Extraction, and CNN should be better than their old counterparts when they are evaluated separately.
%However, the performance of the new pipeline that incorporated both updates is generally unknown until it is actually evaluated.
%For example, the version of Feature Extraction has been updated to 1.0 in the MERGE HEAD, but it is unknown that the updated CNN 0.4 in the HEAD can achieve good accuracy when it applies the new Feature Extraction 1.0. When we consider pipeline performance, we would consider the overall performance when different components assemble as a whole pipeline, rather than the individual performance of the components. We can not guarantee that an updated component in a pipeline is still performing well after it is merged with another pipeline, because it involves the updates of other components. In other words, the solution space is dependent on the pipeline search space which is usually huge, and an unknown solution space could have multiple local optima."
}

\comments{D5}{
On page 5, the search space of a component on a branch is defined. It is said that all pipeline versions
on a branch are considered. But what if a branch has merges in its past? Why do we neglect the versions that occur in those branches? If the reason is to reduce the search space, please say it explicitly.
}

\response{
In the revised paper, we have explicitly stated the reasons why we consider only the versions developed starting from the common ancestor while neglecting the versions before the common ancestor in paragraph 6 of subsection~\textbf{Merge} in Section~\ref{sec: supporting non-linear version history}.

Specifically, the purpose of the development is to improve the pipeline at the common ancestor. 
The versions before the common ancestor are not considered since they could be outdated or irrelevant to the pipeline improvement. 
This helps to reduce the computation time.

% In the revised paper, we have included the above discussion in 

% We have explicitly stated the reasons why we consider only the versions developed starting from the common ancestor while neglecting the versions before the common ancestor. 

% The appended text is located at in Section~\ref{sec: supporting non-linear version history} at the topic \textbf{Merge}:

% "The search space involves all the available component versions developed starting from the common ancestors towards the HEAD and MERGE HEAD. 
% This is based on the assumption that the purpose of the development is to improve the pipeline at the common ancestor.
% Hence, the versions before the common ancestor are ignored since they could be outdated or irrelevant to the pipeline improvement. 
% Moreover, this assumption leads to much reduction of computation time, or otherwise the history before the merge could be too long to be evaluated."
}

\section*{Response to Reviewer \#3}
\comments{D1}{Currently, the evaluation compares MLCask against itself, demonstrating that the optimizations work. This is necessarry but not sufficient.
In the related work section, the authors explain that systems such as MLlib and ModelDB do not support semantic versioning. This may be true, but it does not justify why there is no comparison against those systems. It'd be interesting to understand how MLCask improves performance with respect to an existing baseline. A comparison against these systems is necessary.}

\comments{W1}{Compare against other MLTracking systems in a detailed evaluation. Usability, performance, feature map. Two specific systems come to mind, MLFlow and ModelDB.}

\response{
We have added experiments to compare MLCask with ModelDB and MLflow in terms of run time and storage size in Section~\ref{exp-linear-version}.
Experimental results on the total time, pipeline time composition and cumulative storage space are shown in Fig.~\ref{fig: lv-time}, Fig.~\ref{fig: lv-breakdown}. and Fig.~\ref{fig: lv-storage} respectively.
ModelDB achieves worse performance than MLCask and MLflow because it does not support automatic reuse of intermediate results.
MLCask incurs less pipeline time and storage than MLflow due to its use of version control semantics and the ability to detect incompatibility between components.
}

\comments{D2}{
How much effort does an ML engineer need to invest to benefit from MLCask? With clear benefits, it makes
sense that developers need to commit some effort, but it is hard to distill how much effort this is. A developer would need to describe the metadata of datasets and libraries, but no details about these aspects are given. How hard is it? What does it consist of? And, how likely is it to make a mistake and break the merge operation, for example?
}

\comments{W2}{
Explain clearly how a user would use this system.
}

\response{
The effort that ML engineers need to invest in when they use the system is to prepare the component metafiles and a pipeline metafile. 
We have added more details about the metafiles in paragraph 3 of subsection~\textbf{Component} and paragraph 1 of subsection~\textbf{Pipeline} in Section~\ref{sec: system design} respectively.

% "The mandatory metafile describes the entry point, inputs and outputs, as well as all the essential hyperparameters in running the library. 
% For a library of ML model training, the commonly used hyperparameters could be the learning rate and the maximum number of iterations."

% "A pipeline metafile describes the order of the pipeline components.
% Since the input/output schemas of the components are subject to change during the commits in the development process, the metafile of the components should be separated from the metafile of the pipeline. "
}
%%% ooibc: again, what for?

\comments{D3}{
The authors explain that the system is deployed in a health system, and they use at least 2 pipelines informed by such a deployment. This is great. In general, however, the deployment seems underexploited:
- What's the user experience like? In terms of using the system, interfaces to it, merging experience, etc.
- How exactly did MLCask help address the two challenges of section 2?}

\comments{W3}{The deployment is underexploited. Report on the experience, in particular, as it relates to the design decisions made in the paper. I'd particularly would like to understand what the motivation for the 'merge' functions is, what problems were found in practice that led here.
}

\response{
Through the coordination of a co-author, who is a clinician and Deputy Chief Medical Informatics Officer of the National University Hospital (NUH), we have designed and implemented \system{} to meet the needs of its data scientists and clinicians.

We have added a new Section~\ref{sec: discussion} to report our deployment experience in a hospital.
In this new section, we have explained the three issues we have encountered in the hospital environment: (i) frequent retraining, (ii) needs for branching, and (iii) merge of updated pipelines. 
MLCask is designed for the efficient management of collaborative data analytics pipeline updates that address the three issues.
}

\comments{D4}{
Section 2: the running example is not useful.
}

\response{
The running example in Section~\ref{sec: challenge} is removed with the removal of the original Fig. 1. 
In the revised paper, Fig.~\ref{fig:branch-merge} explains the asynchronous pipeline component update scenario. 
We have added more details and explanation on the asynchronous pipeline component update scenario in subsection~\textbf{Merge} of Section~\ref{sec: supporting non-linear version history}.
}

\comments{D5}{
"For data in relational tables, all the column headers are extracted, standardized, sorted, and then concatenated into a single flat vector." what about non-relational data?
}

\response{
For non-relational data, we can adopt the meta information which determines whether the dataset is compatible with its succeeding libraries that are being used, e.g., shape for image datasets, vocabulary size for text datasets, etc. 
We have included the above discussion in paragraph 3 of Section~\ref{sec: version control of pipeline components}.

}
%%% ooibc: again, what is the point


\comments{D6}{
"existing approaches cannot fulfill the gap when non-linear versioning arises, which is common in ML pipelines where multiple disciplines are involved. " what does 'disciplines' mean here?
}

\response{
We have changed "multiple disciplines" to "multiple user roles" in the revised paper to avoid confusion.
}

\end{multicols}

\twocolumn

\clearpage

==> shepherd_cover_letter.tex <==
\newcommand{\comments}[2]{\noindent\underline{\textbf{Comment #1}}: \emph{#2}}
\newcommand{\response}[1]{\vspace{1mm}\noindent\textbf{RESPONSE}: #1\vspace{1mm}}
\newcommand{\revhighlight}[1]{\emph{\textbf{\uuline{#1}}}}
\pagestyle{empty}
\thispagestyle{empty}

% \newcommand{\question}[1]{}
\newcommand{\question}[1]{{\textcolor{blue}{(#1)}}}

\onecolumn

\centerline{\textbf{\Large Response to Reviewers' Comments}}
\vspace{10mm}

\begin{multicols}{2}
% \raggedcolumns

\setcounter{page}{1}

\noindent To PC co-chairs, meta reviewer, and reviewers:

\vspace{5mm}
Thank you for accepting this manuscript with shepherding.
We have studied the comments carefully and have addressed the concern of clarifying the correctness of the resource efficient approach. In this cover letter, we provide detailed responses to this raised concern.

For ease of reading, we have highlighted the major changes in the revised paper in {\color{blue} blue}.

\section*{Response to Reviewer \#1}
\comments{}{
% The authors addressed most of my concerns. 
% I am not quite happy with regard to my main concern though. 
I had asked about analysis of the correctness of the resource efficient approach. 
The authors do not discuss that in detail. 
They are saying that the approach could lead to the desired results. 
This is not really convincing. 
I had expected some sort of effectiveness comparison. 
% While appreciating the efforts in addressing my other concerns, 
% I think this is an important piece, which has been ignored. 
}
%%% shorten reviewers' comments

\response{
In Section~\ref{exp-pps}, we have added Table I and paragraphs 5 and 6 to clarify the correctness of the resource efficient approach, i.e., the prioritized pipeline search. 

First, the prioritized pipeline search only changes the order of searches without changing the search space. 
Consequently, if the time budget is sufficiently large for searching all the solutions, the prioritized pipeline search will guarantee to obtain the optimal pipeline.

Second, if the time budget is limited, the prioritized pipeline search only searches the most promising pipelines according to the history.
Experimental results show that the prioritized pipeline search finds better pipelines than random search under limited time budget, and the optimal pipeline is more likely to be found in the early searches.
}

\end{multicols}

\twocolumn

\clearpage
